Adaptive LiDAR-Radar Fusion for Outdoor Odometry Across Dense Smoke Conditions

Robust odometry estimation in perceptually degraded environments represents a key challenge in the field of robotics. In this paper, we propose a LiDAR-radar fusion method for robust odometry for adverse environment with LiDAR degeneracy. By comparing the LiDAR point cloud with the radar static point cloud obtained through preprocessing module, it is possible to identify instances of LiDAR degeneracy to overcome perceptual limits. We demonstrate the effectiveness of our method in challenging conditions such as dense smoke, showcasing its ability to reliably estimate odometry and identify/remove dynamic points prone to LiDAR degeneracy.

==> note.tex <==
# Free Notes


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \subfloat[Overlap of two images\label{fig:feature_overlap1}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap.png}
%     }
%     \subfloat[Revloution scan delay\label{fig:feature_overlap2}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap2.png}
% 	}\\
%     \subfloat[Contour and nearest point extraction\label{fig:feature_contour}]{
% 		\includegraphics[width=0.98\columnwidth]{./figs/features.pdf}
% 	}
%     \vspace{-1mm}
%     \caption{(a) In our dataset, certain regions remain un-updated due to the low update rate. An accumulation in these overlapping areas could lead to unexpected convergence behaviors. (b) Given that radar imagery inherently constitutes scan-rotated images, there exists a discrepancy between the commencement and conclusion of the scans, primarily attributed to temporal lags. This discrepancy is especially pronounced during sharp rotational movements. (c) Initially, we delineate the contour, subsequently identifying proximal points to ensure consideration extends beyond just the central points.}
%     \label{fig:feature}
%     \vspace{-5mm}
% \end{figure}


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \includegraphics[width=0.98\columnwidth]{./figs/fig3.pdf}
%     \vspace{-1mm}
%     \caption{Concept of the LodeStar Descriptor. From the primary radar imagery, we compute a radial intensity vector for every $\theta$. Each of these vectors is subsequently integrated to constitute a column within the integrated radial intensity matrix. By iterating this process over a period of 2$\pi$, we synthesize the final descriptor.}
%     \label{fig:lodestar}
%     \vspace{-5mm}
% \end{figure}


root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-48-03_minmax/recall_rates.csv 
STHEREO-SNU, 56.73, 74.61, 80.08, 84.90
STHEREO-valley, 83.60, 96.46, 98.71, 99.36
vivid-urban, 92.22, 98.13, 99.22, 99.69
vivid-city, 92.02, 96.55, 98.17, 98.99

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-49-24_histeq/recall_rates.csv 
STHEREO-SNU, 63.02, 79.35, 84.41, 88.33
STHEREO-valley, 75.88, 89.39, 94.53, 96.14
vivid-urban, 91.91, 98.29, 98.91, 99.69
vivid-city, 89.25, 97.84, 98.78, 99.19

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-50-31_minmax_gridwise_8x8/recall_rates.csv 
STHEREO-SNU, 53.55, 75.02, 81.31, 86.69
STHEREO-valley, 50.80, 71.38, 76.85, 81.99
vivid-urban, 88.49, 96.58, 98.76, 99.53
vivid-city, 91.62, 96.08, 97.50, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-51-45_minmax_gridwise_message_passing_8x8_mean_3/recall_rates.csv 
STHEREO-SNU, 61.80, 79.51, 85.22, 89.80
STHEREO-valley, 87.78, 97.43, 98.71, 99.04
vivid-urban, 93.78, 98.44, 99.07, 99.84
vivid-city, 92.97, 96.08, 97.57, 98.51

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-53-10_minmax_gridwise_message_passing_8x8_mean_5/recall_rates.csv 
STHEREO-SNU, 60.33, 77.80, 81.80, 87.27
STHEREO-valley, 90.03, 96.78, 98.07, 99.36
vivid-urban, 94.40, 99.22, 99.38, 99.84
vivid-city, 91.35, 96.42, 97.70, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-54-42_minmax_gridwise_message_passing_16x16_mean_3/recall_rates.csv 
STHEREO-SNU, 65.71, 80.24, 84.33, 89.06
STHEREO-valley, 76.21, 91.00, 95.18, 96.78
vivid-urban, 92.07, 97.51, 99.07, 100.00
vivid-city, 90.40, 96.35, 97.77, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-55-56_minmax_gridwise_message_passing_16x16_mean_5/recall_rates.csv 
STHEREO-SNU, 59.67, 77.55, 83.51, 88.24
STHEREO-valley, 76.85, 90.03, 95.50, 97.43
vivid-urban, 89.27, 97.20, 99.07, 99.84
vivid-city, 90.94, 95.47, 97.63, 98.58

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-57-11_minmax_gridwise_message_passing_16x16_mean_7/recall_rates.csv 
STHEREO-SNU, 60.90, 78.94, 84.90, 88.82
STHEREO-valley, 78.46, 93.89, 97.43, 99.36
vivid-urban, 90.82, 97.67, 99.38, 99.84
vivid-city, 90.80, 96.15, 97.90, 98.99

